Towards Cross-Lingual Explanation of Artwork in Large-scale Vision Language Models

As the performance of Large-scale Vision Language Models (LVLMs) improves, they are increasingly capable of responding in multiple languages, and there is an expectation that the demand for explanations generated by LVLMs will grow. However, pre-training of Vision Encoder and the integrated training of LLMs with Vision Encoder are mainly conducted using English training data, leaving it uncertain whether LVLMs can completely handle their potential when generating explanations in languages other than English. In addition, multilingual QA benchmarks that create datasets using machine translation have cultural differences and biases, remaining issues for use as evaluation tasks. To address these challenges, this study created an extended dataset in multiple languages without relying on machine translation. This dataset that takes into account nuances and country-specific phrases was then used to evaluate the generation explanation abilities of LVLMs. Furthermore, this study examined whether Instruction-Tuning in resource-rich English improves performance in other languages. Our findings indicate that LVLMs perform worse in languages other than English compared to English. In addition, it was observed that LVLMs struggle to effectively manage the knowledge learned from English data. Our dataset is available at https://huggingface.co/datasets/naist-nlp/MultiExpArt

==> results/a5-misc.tex <==
\begin{table*}[t]
\centering
\resizebox{0.8\textwidth}{!}{
\footnotesize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}ccccccccc@{}} 
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Input}} & \multirow{2}{*}{Output} & \multirow{2}{*}{LVLM} & \multirow{2}{*}{BLEU} & \multicolumn{3}{c}{ROUGE} & \multirow{2}{*}{BertScore} \\
\cmidrule(lr){5-7}
& & & & 1 & 2 & L & &\\
\midrule

en & en & LLaVA-NeXT & 0.01 & \textbf{0.28} & 0.06 & 0.16 & 0.82 \\ 
en & en & LLaVA-NeXT (FT) & 0.03 & 0.21 & 0.08 & 0.16 & 0.82 \\ 
en & en & Qwen-VL & 0.01 & 0.26 & 0.06 & 0.16 & 0.82 \\ 
en & en & Qwen-VL (FT) & \textbf{0.05} & 0.25 & \textbf{0.09} & \textbf{0.19} & 0.82 \\ 
en & en & mPLUG-Owl2 & 0.01 & 0.26 & 0.05 & 0.15 & \textbf{0.82} \\ 
en & en & Phi-3 & 0.01 & 0.22 & 0.04 & 0.13 & 0.82 \\ 
en & en & XComposer2 & 0.01 & 0.27 & 0.06 & 0.15 & 0.82 \\ 
\midrule
en & es & LLaVA-NeXT & \textbf{0.01 (\textcolor{blue}{-0.01)}} & \textbf{0.28 (\textcolor{blue}{-0.00)}} & \textbf{0.06 (\textcolor{blue}{-0.00)}} & \textbf{0.16 (\textcolor{red}{+0.00)}} & 0.73 (\textcolor{blue}{-0.09}) \\ 
en & es & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.05 (\textcolor{blue}{-0.16}) & 0.01 (\textcolor{blue}{-0.07}) & 0.04 (\textcolor{blue}{-0.12}) & 0.78 (\textcolor{blue}{-0.04}) \\ 
en & es & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.21 (\textcolor{blue}{-0.05}) & 0.04 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.03}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
en & es & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.03 (\textcolor{blue}{-0.22}) & 0.00 (\textcolor{blue}{-0.09}) & 0.03 (\textcolor{blue}{-0.17}) & 0.77 (\textcolor{blue}{-0.05}) \\ 
en & es & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.22 (\textcolor{blue}{-0.04}) & 0.04 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.03}) & \textbf{0.80 (\textcolor{blue}{-0.02)}} \\ 
en & es & Phi-3 & 0.00 (\textcolor{blue}{-0.00}) & 0.19 (\textcolor{blue}{-0.03}) & 0.04 (\textcolor{blue}{-0.01}) & 0.12 (\textcolor{blue}{-0.02}) & 0.79 (\textcolor{blue}{-0.02}) \\ 
en & es & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.19 (\textcolor{blue}{-0.08}) & 0.04 (\textcolor{blue}{-0.02}) & 0.12 (\textcolor{blue}{-0.03}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
\midrule
es & en & LLaVA-NeXT & 0.00 (\textcolor{blue}{-0.01}) & \textbf{0.21 (\textcolor{blue}{-0.07)}} & 0.04 (\textcolor{blue}{-0.02}) & 0.13 (\textcolor{blue}{-0.03}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
es & en & LLaVA-NeXT (FT) & 0.01 (\textcolor{blue}{-0.03}) & 0.13 (\textcolor{blue}{-0.08}) & 0.04 (\textcolor{blue}{-0.05}) & 0.10 (\textcolor{blue}{-0.07}) & 0.81 (\textcolor{blue}{-0.01}) \\ 
es & en & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.15 (\textcolor{blue}{-0.11}) & 0.04 (\textcolor{blue}{-0.02}) & 0.11 (\textcolor{blue}{-0.05}) & \textbf{0.82 (\textcolor{blue}{-0.00)}} \\ 
es & en & Qwen-VL (FT) & \textbf{0.01 (\textcolor{blue}{-0.04)}} & 0.21 (\textcolor{blue}{-0.04}) & \textbf{0.05 (\textcolor{blue}{-0.04)}} & \textbf{0.15 (\textcolor{blue}{-0.05)}} & 0.82 (\textcolor{blue}{-0.00}) \\ 
es & en & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.16 (\textcolor{blue}{-0.10}) & 0.04 (\textcolor{blue}{-0.02}) & 0.11 (\textcolor{blue}{-0.04}) & 0.82 (\textcolor{blue}{-0.00}) \\ 
es & en & Phi-3 & 0.00 (\textcolor{blue}{-0.01}) & 0.18 (\textcolor{blue}{-0.04}) & 0.03 (\textcolor{blue}{-0.01}) & 0.12 (\textcolor{blue}{-0.02}) & 0.80 (\textcolor{blue}{-0.01}) \\ 
es & en & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.13}) & 0.03 (\textcolor{blue}{-0.03}) & 0.09 (\textcolor{blue}{-0.06}) & 0.81 (\textcolor{blue}{-0.01}) \\ 
\midrule
es & es & LLaVA-NeXT & \textbf{0.01 (\textcolor{blue}{-0.01)}} & \textbf{0.29 (\textcolor{red}{+0.01)}} & \textbf{0.07 (\textcolor{red}{+0.00)}} & \textbf{0.16 (\textcolor{blue}{-0.00)}} & \textbf{0.81 (\textcolor{blue}{-0.01)}} \\ 
es & es & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.21 (\textcolor{red}{+0.00}) & 0.04 (\textcolor{blue}{-0.04}) & 0.14 (\textcolor{blue}{-0.02}) & 0.79 (\textcolor{blue}{-0.02}) \\ 
es & es & Qwen-VL & 0.01 (\textcolor{blue}{-0.01}) & 0.24 (\textcolor{blue}{-0.03}) & 0.05 (\textcolor{blue}{-0.01}) & 0.14 (\textcolor{blue}{-0.02}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
es & es & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.04 (\textcolor{blue}{-0.21}) & 0.01 (\textcolor{blue}{-0.09}) & 0.04 (\textcolor{blue}{-0.16}) & 0.76 (\textcolor{blue}{-0.06}) \\ 
es & es & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.00}) & 0.22 (\textcolor{blue}{-0.03}) & 0.05 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.03}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
es & es & Phi-3 & 0.01 (\textcolor{blue}{-0.00}) & 0.26 (\textcolor{red}{+0.04}) & 0.05 (\textcolor{red}{+0.01}) & 0.15 (\textcolor{red}{+0.02}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
es & es & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.14}) & 0.03 (\textcolor{blue}{-0.03}) & 0.08 (\textcolor{blue}{-0.07}) & 0.79 (\textcolor{blue}{-0.03}) \\ 
\midrule
en & fr & LLaVA-NeXT & \textbf{0.00 (\textcolor{blue}{-0.01)}} & \textbf{0.21 (\textcolor{blue}{-0.07)}} & \textbf{0.04 (\textcolor{blue}{-0.02)}} & \textbf{0.12 (\textcolor{blue}{-0.04)}} & 0.79 (\textcolor{blue}{-0.02}) \\ 
en & fr & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.06 (\textcolor{blue}{-0.15}) & 0.01 (\textcolor{blue}{-0.07}) & 0.05 (\textcolor{blue}{-0.12}) & 0.78 (\textcolor{blue}{-0.04}) \\ 
en & fr & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.18 (\textcolor{blue}{-0.08}) & 0.03 (\textcolor{blue}{-0.03}) & 0.11 (\textcolor{blue}{-0.05}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
en & fr & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.03 (\textcolor{blue}{-0.23}) & 0.00 (\textcolor{blue}{-0.09}) & 0.02 (\textcolor{blue}{-0.17}) & 0.77 (\textcolor{blue}{-0.05}) \\ 
en & fr & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.19 (\textcolor{blue}{-0.06}) & 0.03 (\textcolor{blue}{-0.02}) & 0.11 (\textcolor{blue}{-0.04}) & \textbf{0.80 (\textcolor{blue}{-0.02)}} \\ 
en & fr & Phi-3 & 0.00 (\textcolor{blue}{-0.00}) & 0.18 (\textcolor{blue}{-0.03}) & 0.03 (\textcolor{blue}{-0.02}) & 0.11 (\textcolor{blue}{-0.02}) & 0.79 (\textcolor{blue}{-0.02}) \\ 
en & fr & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.16 (\textcolor{blue}{-0.11}) & 0.03 (\textcolor{blue}{-0.03}) & 0.10 (\textcolor{blue}{-0.05}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
\midrule
fr & en & LLaVA-NeXT & 0.00 (\textcolor{blue}{-0.01}) & 0.14 (\textcolor{blue}{-0.14}) & 0.02 (\textcolor{blue}{-0.04}) & 0.08 (\textcolor{blue}{-0.08}) & 0.39 (\textcolor{blue}{-0.42}) \\ 
fr & en & LLaVA-NeXT (FT) & \textbf{0.01 (\textcolor{blue}{-0.03)}} & 0.17 (\textcolor{blue}{-0.04}) & 0.04 (\textcolor{blue}{-0.04}) & 0.13 (\textcolor{blue}{-0.04}) & 0.82 (\textcolor{red}{+0.01}) \\ 
fr & en & Qwen-VL & 0.01 (\textcolor{blue}{-0.01}) & 0.15 (\textcolor{blue}{-0.11}) & 0.03 (\textcolor{blue}{-0.02}) & 0.10 (\textcolor{blue}{-0.06}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
fr & en & Qwen-VL (FT) & 0.01 (\textcolor{blue}{-0.04}) & 0.18 (\textcolor{blue}{-0.07}) & 0.04 (\textcolor{blue}{-0.05}) & 0.13 (\textcolor{blue}{-0.07}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
fr & en & mPLUG-Owl2 & 0.01 (\textcolor{blue}{-0.00}) & \textbf{0.22 (\textcolor{blue}{-0.04)}} & \textbf{0.05 (\textcolor{blue}{-0.01)}} & \textbf{0.14 (\textcolor{blue}{-0.02)}} & \textbf{0.82 (\textcolor{red}{+0.00)}} \\ 
fr & en & Phi-3 & 0.00 (\textcolor{blue}{-0.00}) & 0.17 (\textcolor{blue}{-0.05}) & 0.03 (\textcolor{blue}{-0.01}) & 0.11 (\textcolor{blue}{-0.02}) & 0.80 (\textcolor{blue}{-0.01}) \\ 
fr & en & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.15 (\textcolor{blue}{-0.11}) & 0.03 (\textcolor{blue}{-0.03}) & 0.10 (\textcolor{blue}{-0.05}) & 0.81 (\textcolor{blue}{-0.01}) \\ 
\midrule
fr & fr & LLaVA-NeXT & \textbf{0.01 (\textcolor{blue}{-0.01)}} & \textbf{0.26 (\textcolor{blue}{-0.02)}} & \textbf{0.05 (\textcolor{blue}{-0.01)}} & \textbf{0.13 (\textcolor{blue}{-0.03)}} & \textbf{0.80 (\textcolor{blue}{-0.02)}} \\ 
fr & fr & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.15 (\textcolor{blue}{-0.06}) & 0.03 (\textcolor{blue}{-0.05}) & 0.10 (\textcolor{blue}{-0.06}) & 0.79 (\textcolor{blue}{-0.02}) \\ 
fr & fr & Qwen-VL & 0.01 (\textcolor{blue}{-0.01}) & 0.23 (\textcolor{blue}{-0.03}) & 0.04 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.03}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
fr & fr & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.08 (\textcolor{blue}{-0.18}) & 0.01 (\textcolor{blue}{-0.08}) & 0.06 (\textcolor{blue}{-0.14}) & 0.76 (\textcolor{blue}{-0.05}) \\ 
fr & fr & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.00}) & 0.20 (\textcolor{blue}{-0.06}) & 0.04 (\textcolor{blue}{-0.02}) & 0.11 (\textcolor{blue}{-0.05}) & 0.80 (\textcolor{blue}{-0.03}) \\ 
fr & fr & Phi-3 & 0.01 (\textcolor{blue}{-0.00}) & 0.22 (\textcolor{red}{+0.01}) & 0.04 (\textcolor{blue}{-0.00}) & 0.13 (\textcolor{blue}{-0.00}) & 0.79 (\textcolor{blue}{-0.02}) \\ 
fr & fr & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.15 (\textcolor{blue}{-0.11}) & 0.03 (\textcolor{blue}{-0.02}) & 0.10 (\textcolor{blue}{-0.05}) & 0.79 (\textcolor{blue}{-0.03}) \\ 
\midrule
en & ja & LLaVA-NeXT & \textbf{0.01 (\textcolor{blue}{-0.00)}} & \textbf{0.04 (\textcolor{blue}{-0.24)}} & \textbf{0.01 (\textcolor{blue}{-0.06)}} & \textbf{0.04 (\textcolor{blue}{-0.12)}} & \textbf{0.84 (\textcolor{red}{+0.03)}} \\ 
en & ja & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.01 (\textcolor{blue}{-0.20}) & 0.00 (\textcolor{blue}{-0.08}) & 0.01 (\textcolor{blue}{-0.15}) & 0.73 (\textcolor{blue}{-0.09}) \\ 
en & ja & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.02 (\textcolor{blue}{-0.24}) & 0.00 (\textcolor{blue}{-0.06}) & 0.02 (\textcolor{blue}{-0.14}) & 0.83 (\textcolor{red}{+0.01}) \\ 
en & ja & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.05}) & 0.01 (\textcolor{blue}{-0.24}) & 0.00 (\textcolor{blue}{-0.09}) & 0.01 (\textcolor{blue}{-0.18}) & 0.72 (\textcolor{blue}{-0.10}) \\ 
en & ja & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.02 (\textcolor{blue}{-0.24}) & 0.00 (\textcolor{blue}{-0.05}) & 0.02 (\textcolor{blue}{-0.14}) & 0.83 (\textcolor{red}{+0.01}) \\ 
en & ja & Phi-3 & 0.00 (\textcolor{blue}{-0.00}) & 0.02 (\textcolor{blue}{-0.20}) & 0.00 (\textcolor{blue}{-0.04}) & 0.02 (\textcolor{blue}{-0.12}) & 0.82 (\textcolor{red}{+0.01}) \\ 
en & ja & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.02 (\textcolor{blue}{-0.25}) & 0.00 (\textcolor{blue}{-0.05}) & 0.02 (\textcolor{blue}{-0.13}) & 0.83 (\textcolor{red}{+0.01}) \\ 
\midrule
ja & en & LLaVA-NeXT & \textbf{0.01 (\textcolor{blue}{-0.01)}} & \textbf{0.24 (\textcolor{blue}{-0.04)}} & \textbf{0.05 (\textcolor{blue}{-0.02)}} & \textbf{0.15 (\textcolor{blue}{-0.01)}} & 0.82 (\textcolor{red}{+0.00}) \\ 
ja & en & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.16 (\textcolor{blue}{-0.05}) & 0.03 (\textcolor{blue}{-0.05}) & 0.12 (\textcolor{blue}{-0.04}) & 0.82 (\textcolor{red}{+0.00}) \\ 
ja & en & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.18 (\textcolor{blue}{-0.08}) & 0.04 (\textcolor{blue}{-0.02}) & 0.12 (\textcolor{blue}{-0.04}) & 0.81 (\textcolor{blue}{-0.01}) \\ 
ja & en & Qwen-VL (FT) & 0.01 (\textcolor{blue}{-0.04}) & 0.18 (\textcolor{blue}{-0.07}) & 0.03 (\textcolor{blue}{-0.06}) & 0.12 (\textcolor{blue}{-0.07}) & 0.76 (\textcolor{blue}{-0.06}) \\ 
ja & en & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.18 (\textcolor{blue}{-0.08}) & 0.04 (\textcolor{blue}{-0.02}) & 0.12 (\textcolor{blue}{-0.04}) & 0.82 (\textcolor{blue}{-0.00}) \\ 
ja & en & Phi-3 & 0.00 (\textcolor{blue}{-0.00}) & 0.15 (\textcolor{blue}{-0.07}) & 0.03 (\textcolor{blue}{-0.02}) & 0.09 (\textcolor{blue}{-0.04}) & 0.78 (\textcolor{blue}{-0.03}) \\ 
ja & en & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.20 (\textcolor{blue}{-0.06}) & 0.04 (\textcolor{blue}{-0.02}) & 0.12 (\textcolor{blue}{-0.03}) & \textbf{0.82 (\textcolor{red}{+0.00)}} \\ 
\midrule
ja & ja & LLaVA-NeXT & \textbf{0.02 (\textcolor{red}{+0.01)}} & \textbf{0.09 (\textcolor{blue}{-0.19)}} & 0.02 (\textcolor{blue}{-0.04}) & \textbf{0.08 (\textcolor{blue}{-0.08)}} & \textbf{0.85 (\textcolor{red}{+0.03)}} \\ 
ja & ja & LLaVA-NeXT (FT) & 0.01 (\textcolor{blue}{-0.03}) & 0.07 (\textcolor{blue}{-0.14}) & 0.01 (\textcolor{blue}{-0.07}) & 0.06 (\textcolor{blue}{-0.10}) & 0.82 (\textcolor{red}{+0.00}) \\ 
ja & ja & Qwen-VL & 0.02 (\textcolor{red}{+0.00}) & 0.07 (\textcolor{blue}{-0.19}) & 0.02 (\textcolor{blue}{-0.04}) & 0.07 (\textcolor{blue}{-0.09}) & 0.85 (\textcolor{red}{+0.03}) \\ 
ja & ja & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.01 (\textcolor{blue}{-0.24}) & 0.00 (\textcolor{blue}{-0.09}) & 0.01 (\textcolor{blue}{-0.18}) & 0.74 (\textcolor{blue}{-0.08}) \\ 
ja & ja & mPLUG-Owl2 & 0.01 (\textcolor{red}{+0.00}) & 0.05 (\textcolor{blue}{-0.21}) & 0.01 (\textcolor{blue}{-0.04}) & 0.05 (\textcolor{blue}{-0.11}) & 0.81 (\textcolor{blue}{-0.01}) \\ 
ja & ja & Phi-3 & 0.02 (\textcolor{red}{+0.01}) & 0.07 (\textcolor{blue}{-0.15}) & \textbf{0.03 (\textcolor{blue}{-0.02)}} & 0.07 (\textcolor{blue}{-0.06}) & 0.85 (\textcolor{red}{+0.03}) \\ 
ja & ja & XComposer2 & 0.01 (\textcolor{blue}{-0.01}) & 0.05 (\textcolor{blue}{-0.22}) & 0.02 (\textcolor{blue}{-0.04}) & 0.05 (\textcolor{blue}{-0.10}) & 0.84 (\textcolor{red}{+0.02}) \\ 
\midrule
en & it & LLaVA-NeXT & 0.00 (\textcolor{blue}{-0.01}) & 0.09 (\textcolor{blue}{-0.19}) & 0.01 (\textcolor{blue}{-0.05}) & 0.05 (\textcolor{blue}{-0.11}) & 0.40 (\textcolor{blue}{-0.42}) \\ 
en & it & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.04 (\textcolor{blue}{-0.17}) & 0.01 (\textcolor{blue}{-0.08}) & 0.04 (\textcolor{blue}{-0.13}) & 0.77 (\textcolor{blue}{-0.04}) \\ 
en & it & Qwen-VL & \textbf{0.00 (\textcolor{blue}{-0.01)}} & \textbf{0.14 (\textcolor{blue}{-0.12)}} & \textbf{0.02 (\textcolor{blue}{-0.04)}} & \textbf{0.09 (\textcolor{blue}{-0.07)}} & \textbf{0.80 (\textcolor{blue}{-0.02)}} \\ 
en & it & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.04 (\textcolor{blue}{-0.22}) & 0.01 (\textcolor{blue}{-0.09}) & 0.03 (\textcolor{blue}{-0.16}) & 0.76 (\textcolor{blue}{-0.05}) \\ 
en & it & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.14 (\textcolor{blue}{-0.12}) & 0.02 (\textcolor{blue}{-0.04}) & 0.08 (\textcolor{blue}{-0.07}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
en & it & Phi-3 & 0.00 (\textcolor{blue}{-0.01}) & 0.11 (\textcolor{blue}{-0.11}) & 0.01 (\textcolor{blue}{-0.03}) & 0.07 (\textcolor{blue}{-0.06}) & 0.78 (\textcolor{blue}{-0.03}) \\ 
en & it & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.11 (\textcolor{blue}{-0.15}) & 0.01 (\textcolor{blue}{-0.04}) & 0.08 (\textcolor{blue}{-0.07}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
\midrule
it & en & LLaVA-NeXT & 0.01 (\textcolor{blue}{-0.01}) & \textbf{0.23 (\textcolor{blue}{-0.05)}} & \textbf{0.05 (\textcolor{blue}{-0.02)}} & \textbf{0.14 (\textcolor{blue}{-0.02)}} & 0.81 (\textcolor{blue}{-0.01}) \\ 
it & en & LLaVA-NeXT (FT) & \textbf{0.01 (\textcolor{blue}{-0.02)}} & 0.16 (\textcolor{blue}{-0.05}) & 0.04 (\textcolor{blue}{-0.04}) & 0.12 (\textcolor{blue}{-0.04}) & 0.82 (\textcolor{red}{+0.00}) \\ 
it & en & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.17 (\textcolor{blue}{-0.09}) & 0.04 (\textcolor{blue}{-0.02}) & 0.12 (\textcolor{blue}{-0.04}) & 0.82 (\textcolor{blue}{-0.01}) \\ 
it & en & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.09 (\textcolor{blue}{-0.16}) & 0.02 (\textcolor{blue}{-0.07}) & 0.07 (\textcolor{blue}{-0.13}) & 0.40 (\textcolor{blue}{-0.42}) \\ 
it & en & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.16 (\textcolor{blue}{-0.10}) & 0.03 (\textcolor{blue}{-0.02}) & 0.11 (\textcolor{blue}{-0.04}) & \textbf{0.82 (\textcolor{blue}{-0.00)}} \\ 
it & en & Phi-3 & 0.00 (\textcolor{blue}{-0.01}) & 0.13 (\textcolor{blue}{-0.08}) & 0.02 (\textcolor{blue}{-0.02}) & 0.09 (\textcolor{blue}{-0.04}) & 0.80 (\textcolor{blue}{-0.02}) \\ 
it & en & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.15 (\textcolor{blue}{-0.12}) & 0.03 (\textcolor{blue}{-0.03}) & 0.10 (\textcolor{blue}{-0.05}) & 0.81 (\textcolor{blue}{-0.00}) \\ 
\midrule
it & it & LLaVA-NeXT & \textbf{0.00 (\textcolor{blue}{-0.01)}} & \textbf{0.21 (\textcolor{blue}{-0.07)}} & \textbf{0.02 (\textcolor{blue}{-0.04)}} & \textbf{0.11 (\textcolor{blue}{-0.05)}} & \textbf{0.80 (\textcolor{blue}{-0.02)}} \\ 
it & it & LLaVA-NeXT (FT) & 0.00 (\textcolor{blue}{-0.03}) & 0.13 (\textcolor{blue}{-0.08}) & 0.02 (\textcolor{blue}{-0.07}) & 0.08 (\textcolor{blue}{-0.08}) & 0.79 (\textcolor{blue}{-0.03}) \\ 
it & it & Qwen-VL & 0.00 (\textcolor{blue}{-0.01}) & 0.15 (\textcolor{blue}{-0.11}) & 0.02 (\textcolor{blue}{-0.04}) & 0.09 (\textcolor{blue}{-0.07}) & 0.79 (\textcolor{blue}{-0.03}) \\ 
it & it & Qwen-VL (FT) & 0.00 (\textcolor{blue}{-0.04}) & 0.05 (\textcolor{blue}{-0.21}) & 0.00 (\textcolor{blue}{-0.09}) & 0.03 (\textcolor{blue}{-0.16}) & 0.75 (\textcolor{blue}{-0.07}) \\ 
it & it & mPLUG-Owl2 & 0.00 (\textcolor{blue}{-0.01}) & 0.10 (\textcolor{blue}{-0.16}) & 0.01 (\textcolor{blue}{-0.04}) & 0.06 (\textcolor{blue}{-0.09}) & 0.78 (\textcolor{blue}{-0.04}) \\ 
it & it & Phi-3 & 0.00 (\textcolor{blue}{-0.01}) & 0.14 (\textcolor{blue}{-0.08}) & 0.01 (\textcolor{blue}{-0.03}) & 0.09 (\textcolor{blue}{-0.04}) & 0.78 (\textcolor{blue}{-0.03}) \\ 
it & it & XComposer2 & 0.00 (\textcolor{blue}{-0.01}) & 0.06 (\textcolor{blue}{-0.20}) & 0.01 (\textcolor{blue}{-0.05}) & 0.05 (\textcolor{blue}{-0.11}) & 0.77 (\textcolor{blue}{-0.05}) \\ 
\midrule

\bottomrule
\end{tabular}
}
\caption{Results of LVLMs in Full Task. Bold fonts indicate the best score for that language combination. This result shows that no matter how much the amount of data is increased, the best performance is achieved by having instructions given and output in English. The values are noted next to the output of the difference by the same model in the method with instruction and output in English (\{En\}-\{En\}). \textcolor[HTML]{AD0000}{Red} indicates a higher value than that method; \textcolor[HTML]{1400AD}{blue} indicates a lower value.}

\label{tab:result-score-full}
\end{table*}

